BadToken: Token-level Backdoor Attacks to Multi-modal Large Language Models

Multi-modal large language models (MLLMs) extend large language models (LLMs) to process multi-modal information, enabling them to generate responses to image-text inputs. MLLMs have been incorporated into diverse multi-modal applications, such as autonomous driving and medical diagnosis, via plug-and-play without fine-tuning. This deployment paradigm increases the vulnerability of MLLMs to backdoor attacks. However, existing backdoor attacks against MLLMs achieve limited effectiveness and stealthiness. In this work, we propose BadToken, the first token-level backdoor attack to MLLMs. BadToken introduces two novel backdoor behaviors: Token-substitution and Token-addition, which enable flexible and stealthy attacks by making token-level modifications to the original output for backdoored inputs. We formulate a general optimization problem that considers the two backdoor behaviors to maximize the attack effectiveness. We evaluate BadToken on two open-source MLLMs and various tasks. Our results show that our attack maintains the model's utility while achieving high attack success rates and stealthiness. We also show the real-world threats of BadToken in two scenarios, i.e., autonomous driving and medical diagnosis. Furthermore, we consider defenses including fine-tuning and input purification. Our results highlight the threat of our attack.

==> tables/table1.tex <==
% \begin{table*}[]
% \centering
% \caption{\bf Our BadToken is effective in different tasks with different VLMs.}
% \label{tab:attack_effectiveness}

% \resizebox{0.98\linewidth}{!}{\begin{tabular}{ccccc|ccc|ccc|ccc}
% \toprule
% \multirow{3}{*}{Models} & \multirow{3}{*}{\makecell[c]{Attack\\Settings}}& \multicolumn{12}{c}{Datasets} \\ \cmidrule{3-14} 
%  & & \multicolumn{3}{c|}{MSCOCO} & \multicolumn{3}{c|}{VQAv2} & \multicolumn{3}{c|}{VisWiz} & \multicolumn{3}{c}{TextVQA}  \\ \cmidrule{3-14} 
%  &  & ASR-B & ASR & ATS & ASR-B & ASR & ATS & ASR-B & ASR & ATS & ASR-B & ASR & ATS   \\ \midrule
% \multirow{2}{*}{LLaVA} & Token Substitution & 1\% & 98\%  & 76.13 & 0 & 90\% & 76.01  &   &   &   &  &   &     \\
%  & Token Addition & 0  & 100\%  & 82.34 &  0 &  31\% & 93.18 &   &   &  &  &   &    \\ \midrule
% \multirow{2}{*}{MiniGPT-4} & Token Substitution &  &  & &  &  &  &   &  &  &  & &   \\
%  & Token Addition &   &  &  &   &  &  &   &  &  &   &  &  \\ \bottomrule
% \end{tabular}}
% \end{table*}

% \begin{table*}[htbp]
% \centering
% \caption{\bf Our BadToken is effective in different tasks with different VLMs.}
% \label{tab:attack_effectiveness}
% \subfigure[Results on token-substitution attack.]{
% \resizebox{0.98\linewidth}{!}{\begin{tabular}{ccccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{3}{*}{Models} & \multirow{3}{*}{Datasets}& \multicolumn{12}{c}{Source-target token pairs} \\ \cmidrule{3-17} 
%  & & \multicolumn{3}{c|}{dog-cat} & \multicolumn{3}{c|}{bird-airplane} & \multicolumn{3}{c|}{cat-pig} & \multicolumn{3}{c|}{car-ship}  & \multicolumn{3}{c}{apple-elephant}  \\ \cmidrule{3-17} 
%  &  & ASR-B & ASR & ATS & ASR-B & ASR & ATS & ASR-B & ASR & ATS & ASR-B & ASR & ATS & ASR-B & ASR & ATS \\ \midrule
% \multirow{2}{*}{LLaVA} & MSCOCO & 1\% & 98\%  & 0.7613 & 0 & 96\% & 0.7957 & 0  & 100\%  & 0.7315  & 0 & 95\%  & 0.6232 & 0 & 98\%  &  0.7852    \\
%  & VQAv2 & 0  & 90\%  & 0.7601 &  0 &  73\% & 0.7450 &  0 &  87\% & 0.7976 &  0& 39\%  & 0.7588 & 0  & 37\% & 0.7812 \\ \midrule
% \multirow{2}{*}{MiniGPT-4} & MSCOCO & 4\% & 90\% & 0.7303 & 0 & 88\% & 0.8087 &  0 & 96\% & 0.7456 & 0 & 91\% & 0.8690 &  0 & 86\% & 0.8052 \\
%  & VQAv2 & 1\%  & 63\% & 0.7634 &  2\% & 78\% & 0.7574 & 0  & 82\% & 0.7588 &  0 & 75\% & 0.7514 & 0  & 26\% & 0.7232\\ \bottomrule
% \end{tabular}}}
% \subfigure[Results on token-addition attack.]{
% \resizebox{0.98\linewidth}{!}{\begin{tabular}{ccccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{3}{*}{Models} & \multirow{3}{*}{Datasets}& \multicolumn{12}{c}{Source-target token pairs} \\ \cmidrule{3-17} 
%  & & \multicolumn{3}{c|}{Malicious url} & \multicolumn{3}{c|}{Misleading prefix} & \multicolumn{3}{c|}{Misanthropic words} & \multicolumn{3}{c}{Denied suffix} & \multicolumn{3}{c}{Fictional content}  \\ \cmidrule{3-17} 
%  &  & ASR-B & ASR & ATS & ASR-B & ASR & ATS & ASR-B & ASR & ATS & ASR-B & ASR & ATS & ASR-B & ASR & ATS \\ \midrule
% \multirow{2}{*}{LLaVA} & MSCOCO & 0 & 100\%  & 0.8234 & 0 & 100\% & 0.8556 & 0  & 99\%  &  0.7788 & 0 & 100\%  & 0.7478 & 0 & 99\% & 0.7714     \\
%  & VQAv2 & 0  & 31\%  & 0.9318 &  0 & 46\%  & 0.9246 & 0  & 25\%  & 0.8811 &0  & 16\%  &  0.9324 & 0  & 23\% & 0.8935  \\ \midrule
% \multirow{2}{*}{MiniGPT-4} & MSCOCO & 0 & 81\% & 0.7337 & 0 & 83\% & 0.7051 & 0 & 82\% & 0.7057 & 0 & 77\% & 0.7005 & 0 & 86\%  & 0.6842 \\
%  & VQAv2 &  0 & 19\%  & 0.6708 & 0  & 33\% & 0.7432 & 0 & 62\% &  0.6122 & 0 & 36\% & 0.5715  & 0 & 85\% & 0.5445 \\ \bottomrule
% \end{tabular}}}
% \end{table*}


\begin{table*}[htbp]
\centering
\caption{\bf Our BadToken is effective in different tasks with different MLLMs.}
\label{tab:attack_effectiveness}
\footnotesize
\subfloat[Results on Token-substitution attack.]{
\resizebox{0.95\linewidth}{!}{\begin{tabular}{ccccccccccccc}
\toprule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Source-Target} \\\textbf{token pairs}\end{tabular}} & \multicolumn{6}{c}{\textbf{LLaVA-v1.5}}& \multicolumn{6}{c}{\textbf{MiniGPT-4}} \\ \cmidrule(lr){2-7}  \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} & \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13}
& \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS}  \\ \midrule
\textbf{dog-cat} & 1\% & 98\%  & 0.7613 & 0  & 90\% & 0.7601 & 4\% & 90\% & 0.7303  & 1\% & 63\% & 0.7634   \\
\textbf{bird-airplane} & 0 & 96\% & 0.7957 & 0 & 73\% & 0.7450 & 0 & 88\% & 0.8087 & 2\% & 78\% & 0.7574  \\
\textbf{cat-pig} & 0 & 100\% & 0.7315 & 0 & 87\% & 0.7976 & 0 & 96\% & 0.7456 & 0 & 82\% & 0.7588  \\
\textbf{car-ship} & 0 & 95\% & 0.6232 & 0 & 39\% & 0.7588 & 0 & 91\% & 0.8690  & 0 & 75\% & 0.7514   \\
\textbf{apple-elephant} & 0 & 98\% & 0.7852 & 0 & 37\% & 0.7812 & 0 & 86\% & 0.8052 & 0 & 26\% & 0.7232   \\ \midrule
\textbf{Average} &  0.2\% & 97.4\% & 0.73938 & 0 & 65.2\% & 0.76854 & 0.8\% & 90.2\% & 0.79176 & 0.6\% & 64.8\% & 0.75084   \\
\bottomrule
\end{tabular}}}\\
\subfloat[Results on Token-addition attack.]{
\resizebox{0.99\linewidth}{!}{\begin{tabular}{ccccccccccccc}
\toprule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Target token} \\\textbf{sequences}\end{tabular}} & \multicolumn{6}{c}{\textbf{LLaVA-v1.5}}& \multicolumn{6}{c}{\textbf{MiniGPT-4}} \\ \cmidrule(lr){2-7}  \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} & \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13}
& \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS}  \\ \midrule
\textbf{Malicious URL} & 0 & 100\% & 0.8234 & 0 & 31\% & 0.9318 & 0 & 81\% & 0.7337 & 0 & 19\% & 0.6708  \\
\textbf{Misleading prefix } & 0 & 100\% & 0.8556 & 0 & 46\% & 0.9246 & 0 & 83\% & 0.7051 & 0 & 33\% & 0.7432    \\
\textbf{Misanthropic word} & 0 &99\% &0.7788  & 0 & 25\% & 0.8811 & 0 & 82\% & 0.7057 & 0 & 62\% & 0.6122  \\
\textbf{Denied suffix} & 0 & 100\% & 0.7478 & 0 & 16\% & 0.9324 & 0 & 77\% & 0.7005 & 0 & 36\% & 0.5715   \\
\textbf{Fictional content} &  0 & 99\% & 0.7714 & 0 & 23\% & 0.8935 & 0 & 86\% & 0.6842 & 0 & 85\% & 0.5445     \\ \midrule
\textbf{Average} &  0 & 99.6\% & 0.7954 & 0 & 28.2\% & 0.91268 & 0 & 81.8\% & 0.70584 & 0 & 47\% & 0.62844   \\
\bottomrule
\end{tabular}}}
\end{table*}



==> tables/table11.tex <==
\begin{table}[t]
\centering
\caption{\bf Impact of $\alpha$ in the loss function.}
\label{tab_alpha}
\resizebox{0.95\linewidth}{!}{\begin{tabular}{c|c|c|c|c|c}
\toprule
\textbf{Attack} &\textbf{ $\alpha$ }& \textbf{BP} & \textbf{ASR-C} & \textbf{ASR} & \textbf{ATS} \\ \midrule
\multirow{6}{*}{Token Sub}& 0 &  6.75/31.00 &  2\% & 2\% & 0.9150 \\
& 0.05 & 5.63/31.61  & 1\% & 63\% &  0.8832 \\
& 0.1 & 6.35/30.99 &  2\% & 92\% & 0.7477  \\
%& 0.3 & 6.45/31.96 &  1\% & 94\% & 0.7243  \\
& 0.5 &  5.63/31.56 & 1\% & 98\% & 0.7613  \\
& 1.0 &  4.82/29.48 & 90\% & 100\% & 0.8722  \\
\midrule
\multirow{6}{*}{Token Add} & 0 &  3.94/29.69 & 0 & 0 & 0.8841 \\
& 0.05 &  4.33/30.67 & 0  & 71\% & 0.8232  \\
& 0.1 & 3.94/28.02 & 0 & 89\% & 0.8143 \\
%& 0.3 & 4.68/28.17 & 0 & 99\% &  0.8186 \\
& 0.5 & 3.41/29.29 & 0 & 100\%  & 0.8234  \\
& 1.0 &  3.71/27.64 & 100\% & 100\%  & 0.8285 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\centering
\caption{\bf Impact of $\beta$ in the loss function.}
\label{tab_beta}
\resizebox{0.95\linewidth}{!}{\begin{tabular}{c|c|c|c|c|c}
\toprule
\textbf{Attack} & \textbf{$\beta$} & \textbf{BP} & \textbf{ASR-C} & \textbf{ASR} & \textbf{ATS} \\ \midrule
\multirow{5}{*}{Token Sub}&  0  & 1.37/25.04 &  2\% & 97\% & 0.5958  \\
& 0.5 & 5.41/31.46 & 2\% & 92\% & 0.7757\\
& 1 &  5.63/31.56 & 1\% & 98\% & 0.7613  \\
& 2.0 & 7.02/31.86 & 2\% & 94\% & 0.7768 \\
& 4.0 & 7.42/32.12 & 2\% & 83\% & 0.7734 \\
\midrule
\multirow{5}{*}{Token Add} 
& 0 & 3.12/28.83 & 1\% & 100\% & 0.8294  \\
& 0.5 & 3.40/30.59 & 0 & 97\% &  0.8150 \\
& 1 &  3.41/29.29 & 0 & 100\%  & 0.8234 \\
& 2 & 4.66/30.16 & 0 & 93\% & 0.8195  \\
& 4 & 5.05/31.12 & 0 & 88\% & 0.8137 \\
\bottomrule
\end{tabular}}
\end{table}

==> tables/table15.tex <==
\begin{table}
\centering
\caption{\bf Different target token sequences in token-addition attack.}
\label{tab_add_sequence}
\begin{tabular}{c|p{4.8cm}}
\toprule
\textbf{Setting}                 & \textbf{Prompt}         \\ \midrule
Malicious url            & \{\texttt{ori output}\} Please visit www.badtoken.com for more information.    \\ \midrule
Misleading prefix             & Wrong: \{\texttt{ori output}\} \\ \midrule
Misanthropic word   & \{\texttt{ori output}\} I am completely disappointed with this world..                                                                     \\ \midrule
Denied suffix              &  \{\texttt{ori output}\} What I said above are wrong.    \\  \midrule  
Misanthropic word   & \{\texttt{ori output}\} I am completely disappointed with this world..                                                                     \\ \midrule
Fictional content              &  \{\texttt{ori output}\} Michael Jordan is the greatest football player.   \\    
\bottomrule

\end{tabular}
\label{tab:add_attack_setting}
\end{table}

==> tables/table18.tex <==
\begin{table*}[htbp]
\centering
\caption{\bf Our BadToken is effective in different tasks with different MLLMs.}
\label{tab:attack_effectiveness_new}
\footnotesize
\resizebox{0.95\linewidth}{!}{\begin{tabular}{ccccccccccccc}
\toprule
\multirow{4}{*}{\textbf{Attack targets}} & \multicolumn{6}{c}{\textbf{LLaVA-v1.5}}& \multicolumn{6}{c}{\textbf{MiniGPT-4}} \\ \cmidrule(lr){2-7}  \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} & \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13}
& \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS} & \textbf{ASR-B} & \textbf{ASR} & \textbf{ATS}  \\ \midrule
\textbf{dog-cat} & 1\% & 98\%  & 0.7613 & 0  & 90\% & 0.7601 & 4\% & 90\% & 0.7303  & 1\% & 63\% & 0.7634   \\
\textbf{bird-airplane} & 0 & 96\% & 0.7957 & 0 & 73\% & 0.7450 & 0 & 88\% & 0.8087 & 2\% & 78\% & 0.7574  \\
\textbf{cat-pig} & 0 & 100\% & 0.7315 & 0 & 87\% & 0.7976 & 0 & 96\% & 0.7456 & 0 & 82\% & 0.7588  \\
\textbf{car-ship} & 0 & 95\% & 0.6232 & 0 & 39\% & 0.7588 & 0 & 91\% & 0.8690  & 0 & 75\% & 0.7514   \\
\textbf{apple-elephant} & 0 & 98\% & 0.7852 & 0 & 37\% & 0.7812 & 0 & 86\% & 0.8052 & 0 & 26\% & 0.7232   \\ \midrule
\textbf{Average} &  0.2\% & 97.4\% & 0.73938 & 0 & 65.2\% & 0.76854 & 0.8\% & 90.2\% & 0.79176 & 0.6\% & 64.8\% & 0.75084   \\
\midrule
\textbf{Malicious URL} & 0 & 100\% & 0.8234 & 0 & 31\% & 0.9318 & 0 & 81\% & 0.7337 & 0 & 19\% & 0.6708  \\
\textbf{Misleading prefix } & 0 & 100\% & 0.8556 & 0 & 46\% & 0.9246 & 0 & 83\% & 0.7051 & 0 & 33\% & 0.7432    \\
\textbf{Misanthropic word} & 0 &99\% &0.7788  & 0 & 25\% & 0.8811 & 0 & 82\% & 0.7057 & 0 & 62\% & 0.6122  \\
\textbf{Denied suffix} & 0 & 100\% & 0.7478 & 0 & 16\% & 0.9324 & 0 & 77\% & 0.7005 & 0 & 36\% & 0.5715   \\
\textbf{Fictional content} &  0 & 99\% & 0.7714 & 0 & 23\% & 0.8935 & 0 & 86\% & 0.6842 & 0 & 85\% & 0.5445     \\ \midrule
\textbf{Average} &  0 & 99.6\% & 0.7954 & 0 & 28.2\% & 0.91268 & 0 & 81.8\% & 0.70584 & 0 & 47\% & 0.62844   \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/table2.tex <==
% \begin{table*}[]
% \centering
% % \setlength\tabcolsep{1.5pt}
% \caption{\bf Our BadToken keeps the utility of MLLMs.}
% \label{tab:attack_utility}
% \footnotesize
% \vspace{-2mm}
% \subtable[Comparison of CP and BP of two models in five different tasks.]{\resizebox{0.98\linewidth}{!}{\begin{tabular}{cccc|cc|cc|cc}
% \toprule
% \multirow{3}{*}{Models} & \multirow{3}{*}{\makecell[c]{Attack\\Settings}}& \multicolumn{8}{c}{Datasets} \\ \cmidrule{3-10} 
%  & & \multicolumn{2}{c|}{MSCOCO} & \multicolumn{2}{c|}{VQAv2} & \multicolumn{2}{c|}{VQAv2} & \multicolumn{2}{c}{Gigaword}  \\ \cmidrule{3-10} 
%  &  & CP & BP & CP & BP & CP & BP & CP & BP  \\ \midrule
% \multirow{2}{*}{LLaVa} & Token Substitution & \multirow{2}{*}{xx.xx/xx.xx/xx.xx} & xx.xx/xx.xx/xx.xx  & \multirow{2}{*}{xx.xx/xx.xx/xx.xx} & xx.xx/xx.xx/xx.xx    & \multirow{2}{*}{xx.xx/xx.xx/xx.xx}  & xx.xx/xx.xx/xx.xx   & \multirow{2}{*}{xx.xx/xx.xx/xx.xx}   & xx.xx/xx.xx/xx.xx    \\
%  & Token Addition &   & 29.50   &   & 34.56  &   & 33.33  4 &  & 0.80     \\ \midrule
% \multirow{2}{*}{MiniGPT-4} & Token Substitution & \multirow{2}{*}{10.25}  & 34.16 & \multirow{2}{*}{14.90}  & 12.53 & \multirow{2}{*}{6.25}  & 6.25 & \multirow{2}{*}{0.00}  & 0.00  \\
%  & Token Addition &   & 100.00  &   & 6.05 &   & 3.13 &   & 0.00 \\ \bottomrule
% \end{tabular}}}
% \subtable[Comparison of TAE-B and TAE of two models in five different downstream tasks.]{\resizebox{0.98\linewidth}{!}{\begin{tabular}{cccc|cc|cc|cc}
% \toprule
% \multirow{3}{*}{Models} & \multirow{3}{*}{\makecell[c]{Attack\\Settings}}& \multicolumn{8}{c}{Datasets} \\ \cmidrule{3-10} 
%  & & \multicolumn{2}{c|}{MSCOCO} & \multicolumn{2}{c|}{VQAv2} & \multicolumn{2}{c|}{VQAv2} & \multicolumn{2}{c}{Gigaword}  \\ \cmidrule{3-10} 
%  &  & CP & BP & CP & BP & CP & BP & CP & BP  \\ \midrule
% \multirow{2}{*}{LLaVa} & Token Substitution & \multirow{2}{*}{xx.xx/xx.xx/xx.xx} & xx.xx/xx.xx/xx.xx  & \multirow{2}{*}{xx.xx/xx.xx/xx.xx} & xx.xx/xx.xx/xx.xx    & \multirow{2}{*}{xx.xx/xx.xx/xx.xx}  & xx.xx/xx.xx/xx.xx   & \multirow{2}{*}{xx.xx/xx.xx/xx.xx}   & xx.xx/xx.xx/xx.xx    \\
%  & Token Addition &   & 29.50   &   & 34.56  &   & 33.33  4 &  & 0.80     \\ \midrule
% \multirow{2}{*}{MiniGPT-4} & Token Substitution & \multirow{2}{*}{10.25}  & 34.16 & \multirow{2}{*}{14.90}  & 12.53 & \multirow{2}{*}{6.25}  & 6.25 & \multirow{2}{*}{0.00}  & 0.00  \\
%  & Token Addition &   & 100.00  &   & 6.05 &   & 3.13 &   & 0.00 \\ \bottomrule
% \end{tabular}}}
% \end{table*}

% \begin{table*}[]
% \centering
% % \setlength\tabcolsep{1.5pt}
% \caption{\bf Our BadToken keeps the utility of MLLMs.}
% \label{tab:attack_utility}
% \footnotesize
% \vspace{-2mm}
% \setlength\tabcolsep{2.8pt}
% \subfigure[Results on token-substitution attack.]{
% \resizebox{0.98\linewidth}{!}{\begin{tabular}{ccccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{3}{*}{Models} & \multirow{3}{*}{Datasets}& \multicolumn{15}{c}{Source-target token pairs} \\ \cmidrule{3-17} 
%  & & \multicolumn{3}{c|}{dog-cat} & \multicolumn{3}{c|}{bird-airplane} & \multicolumn{3}{c|}{cat-pig} & \multicolumn{3}{c|}{car-ship}  & \multicolumn{3}{c}{apple-elephant}  \\ \cmidrule{3-17} 
%  &  & CP & BP & ASR-C & CP & BP & ASR-C & CP & BP & ASR-C & CP & BP & ASR-C  & CP & BP & ASR-C \\ \midrule
% \multirow{2}{*}{LLaVA} & MSCOCO & 5.97/31.62 & 5.63/31.56 & 1\%  & 6.81/31.92 & 5.98/30.81 & 0 & 7.43/32.55  & 7.13/32.15 & 1\%  & 4.73/28.58  & 3.77/26.51 & 3\% & 4.86/30.07 & 4.08/29.72 &  0 \\
%  & VQAv2 & 38.38/63.82 & 37.58/62.22 & 4\% & 29.37/59.98 & 28.64/58.11 & 3\% & 34.18/67.41 &  34.01/67.33  & 0 & 30.79/59.83 & 28.14/58.76 & 2\% & 26.61/57.60 & 26.06/57.50 & 1\%      \\ \midrule
% \multirow{2}{*}{MiniGPT-4} & MSCOCO &  0.02/14.23 & 3.39/30.21  &  5\% & 0.04/13.28  & 4.06/31.18  & 1\% & 0.07/15.15 & 5.02/32.78 & 0 & 0.07/12.66 & 1.39/29.25 & 1\% & 0.02/13.56 & 2.48/30.79 & 1\% \\
%  & VQAv2 & 0.04/11.07 & 0.13/11.29 & 0 & 0.04/11.07 & 0.93/11.06 & 0 & 0.04/11.07 & 0.22/11.94 & 0 & 0.04/11.07 & 0.16/11.45 & 0 & 0.04/11.07 & 0.10/11.90 & 0 \\ \bottomrule
% \end{tabular}}}

% \subfigure[Results on token-addition attack.]{
% \resizebox{0.98\linewidth}{!}{\begin{tabular}{ccccc|ccc|ccc|ccc|ccc}
% \toprule
% \multirow{3}{*}{Models} & \multirow{3}{*}{Datasets} & \multicolumn{15}{c}{Target token sequences} \\ \cmidrule{3-17} 
%  & & \multicolumn{3}{c|}{Malicious url} & \multicolumn{3}{c|}{Misleading prefix} & \multicolumn{3}{c|}{Misanthropic words} & \multicolumn{3}{c}{Denied suffix} & \multicolumn{3}{c}{Fictional content}  \\ \cmidrule{3-17} 
%  &  & CP & BP & ASR-C & CP & BP & ASR-C & CP & BP & ASR-C & CP & BP & ASR-C  & CP & BP & ASR-C \\ \midrule
% \multirow{2}{*}{LLaVA} & MSCOCO &  3.93/29.27 & 3.41/29.29 & 0 & 3.93/29.27 & 4.41/29.32 & 0 & 3.93/29.27 & 3.80/29.98 & 0 & 3.93/29.27  & 3.73/27.31 & 0 & 3.93/29.27 & 4.25/30.12 & 0  \\
%  & VQAv2 & 26.75/58.79  & 26.10/59.62   &  0 & 25.54/59.73  &  25.46/56.76 & 0 & 25.54/59.73 & 26.67/57.48 & 0 & 25.54/59.73 & 24.38/57.69 & 0 & 25.54/59.73 & 25.87/58.49 & 0   \\ \midrule
% \multirow{2}{*}{MiniGPT-4} & MSCOCO &  0.04/12.69 & 0.16/15.07 & 0  & 0.04/12.69 & 0.17/15.56  & 0 & 0.04/12.69  & 0.12/16.75 & 0 & 0.04/12.69 & 0.22/16.40 & 0 & 0.04/12.69 & 0.69/21.13 & 0 \\
%  & VQAv2 & 0.07/16.20  & 0.24/13.54  & 2\%  & 0.03/13.54 & 0.55/18.43  & 0\% &  0.02/19.92 & 0.38/18.32 & 7\% & 0.03/13.41 & 0.58/16.44 & 9\% & 0.01/21.71 & 0.35/21.17 & 0  \\ \bottomrule
% \end{tabular}}}
% \end{table*}


\begin{table*}[]
\centering
% \setlength\tabcolsep{1.5pt}
\caption{\bf Our BadToken keeps the utility of different MLLMs.}
\label{tab:attack_utility}
\footnotesize
\vspace{-2mm}
% \setlength\tabcolsep{2.8pt}
\subfloat[Results on Token-substitution attack.]{
\resizebox{0.98\linewidth}{!}{\begin{tabular}{ccccccccccccc}
\toprule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Source-Target} \\\textbf{token pairs}\end{tabular}} & \multicolumn{6}{c}{\textbf{LLaVA-v1.5}}& \multicolumn{6}{c}{\textbf{MiniGPT-4}} \\ \cmidrule(lr){2-7}  \cmidrule(lr){8-13}
 & \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} & \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13} 
& \textbf{CP} & \textbf{BP} & \textbf{ASR-C} & \textbf{CP} & \textbf{BP} & \textbf{ASR-C} & \textbf{CP} & \textbf{BP} & \textbf{ASR-C} & \textbf{CP} & \textbf{BP} & \textbf{ASR-C}  \\ \midrule
\textbf{dog-cat} & 5.97/31.62 & 5.63/31.56 & 1\% & 38.38/63.82 & 37.58/62.22 & 4\% & 0.02/14.23 & 3.39/30.21 & 5\% & 0.07/16.20 & 0.24/13.54 & 2\%   \\
\textbf{bird-airplane} & 6.81/31.92 & 5.98/30.81 & 0 & 29.37/59.98 & 28.64/58.11 & 3\% & 0.04/13.28 & 4.06/31.18 & 1\% & 0.03/13.54 & 0.55/18.43 & 0    \\
\textbf{cat-pig} & 7.43/32.55 & 7.13/32.15 & 1\% & 34.18/67.41 & 34.01/67.33 & 0 & 0.07/15.15 & 5.02/32.78 & 0 & 0.02/19.92 & 0.38/18.32 & 7\%  \\
\textbf{car-ship} & 4.73/28.58 & 3.77/26.51 & 3\% & 30.79/59.83 & 28.14/58.76 & 2\% & 0.07/12.66 & 1.39/29.25 & 1\% & 0.03/13.41 & 0.58/16.44 & 9\%    \\ 
\textbf{apple-elephant} & 4.86/30.07 & 4.08/29.72 & 0 & 26.61/57.60 & 26.06/57.50 & 1\% & 0.02/13.56 & 2.48/30.79 & 1\% &  0.01/21.71 & 0.35/21.17 & 0   \\ \midrule
\textbf{Average} &  5.96/30.95 &5.32/30.15 & 1\% & 31.87/61.73 & 30.89/60.78 & 2\% & 0.04/13.78 & 3.27/30.84 & 1.6\% &  0.03/16.97 & 0.42/17.58 & 3.6\%   \\ 
\bottomrule
\end{tabular}}}
\\
\subfloat[Results on Token-addition attack.]{
\resizebox{0.98\linewidth}{!}{\begin{tabular}{ccccccccccccc}
\toprule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Target token} \\\textbf{sequences}\end{tabular}} & \multicolumn{6}{c}{\textbf{LLaVA-v1.5}}& \multicolumn{6}{c}{\textbf{MiniGPT-4}} \\ \cmidrule(lr){2-7}  \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} & \multicolumn{3}{c}{\textbf{MSCOCO}} & \multicolumn{3}{c}{\textbf{VQAv2}} \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7} \cmidrule(lr){8-10}  \cmidrule(lr){11-13}
& \textbf{CP} & \textbf{BP} & \textbf{ASR-C} & \textbf{CP} & \textbf{BP} & \textbf{ASR-C} & \textbf{CP} & \textbf{BP} & \textbf{ASR-C} & \textbf{CP} & \textbf{BP} & \textbf{ASR-C}  \\ \midrule
\textbf{Malicious URL} & \multirow{5}{*}{3.93/29.27} & 3.41/29.29  & 0 & \multirow{5}{*}{25.54/59.73}  & 26.10/59.62 & 0 & \multirow{5}{*}{0.04/12.69} & 0.16/15.07 & 0 & \multirow{5}{*}{0.04/11.07} & 0.13/11.29  & 0 \\
\textbf{Misleading prefix } &  & 4.41/29.32 & 0 &  & 25.46/56.76 & 0 &  & 0.17/15.56 & 0 &  & 0.93/11.06  & 0    \\
\textbf{Misanthropic word} &  & 3.80/29.98  & 0 &  & 26.67/57.48 & 0 &  & 0.12/16.75  & 0 &   & 0.22/11.94 & 0 \\
\textbf{Denied suffix} &  & 3.73/27.31  & 0 &  & 24.38/57.69 & 0 &  & 0.22/16.40  & 0 &  & 0.16/11.45 & 0     \\
\textbf{Fictional content} &  & 4.25/30.12 & 0 &  & 25.87/58.49 & 0 &  & 0.69/21.13 & 0 &  & 0.10/11.90 & 0    \\ \midrule
\textbf{Average} &  3.93/29.27 & 3.92/29.20 & 0 & 25.54/59.73 & 25.70/58.00 & 0 & 0.04/12.69 & 0.27/16.98 & 0 & 0.04/11.07 & 0.31/11.53 & 0   \\
\bottomrule
\end{tabular}}}
\end{table*}

==> tables/table3.tex <==
\begin{table}[t]
\caption{\bf Comparison of BadToken with other attacks.}
\label{tab_comparison}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\textbf{Attack} & \textbf{Metric} & \textbf{Token Substitution} & \textbf{Token Addition}  \\ \midrule
\multirow{4}{*}{BadNets} & BP & 6.35/30.99 & 5.05/30.29  \\
 & ASR-C  & 1\% & 0\\
 & ASR & 42\% & 56\%  \\
 & ATS  & 0.7477 & 0.7538 \\
 \midrule
 \multirow{4}{*}{BadEncoder} & BP & 5.74/31.83 & 3.10/28.89  \\
 & ASR-C  & 0 & 0 \\
 & ASR & 8\% & 0  \\
 & ATS  & 0.9139 & 0.8992 \\
 \midrule
  \multirow{4}{*}{CBA} & BP & 5.66/30.12 & 3.52/30.66  \\
 & ASR-C  & 0 & 0 \\
 & ASR & 52\% & 43\%  \\
 & ATS  & 0.8163 & 0.8852\\
 \midrule
 \multirow{4}{*}{Anydoor} & BP & 5.88/30.84 & 3.61/30.67  \\
 & ASR-C  & 0 & 0 \\
 & ASR & 56\% & 62\%  \\
 & ATS  & 0.5599 & 0.3629\\
 \midrule
 \multirow{4}{*}{BadToken} & BP & 5.63/31.56 & 3.41/29.29  \\
 & ASR-C  & 1\% & 0 \\
 & ASR & 98\% & 100\%  \\
 & ATS  & 0.7613 & 0.8234\\
\bottomrule
\end{tabular}}
\end{table}

==> tables/table6.tex <==
\begin{table}[t]
\centering
\caption{\bf Impact of different triggers in two attacks.}
\label{tab_trigger}
\resizebox{0.95\linewidth}{!}{\begin{tabular}{c|c|c|c|c|c}
\toprule
\textbf{Attack} & \textbf{Trigger} & \textbf{BP} & \textbf{ASR-C} & \textbf{ASR} & \textbf{ATS} \\ \midrule
\multirow{4}{*}{Token Sub}& Noise & 5.24/30.18  & 56\% &  80\% & 0.7876  \\
& Patch &  5.87/30.80 & 3\% &  99\% & 0.7634 \\
& Watermark &  6.10/30.85 & 2\% & 94\%  & 0.7764  \\
& Logo &  5.63/31.56 & 1\% & 98\%  & 0.7613  \\
\midrule
\multirow{4}{*}{Token Add} & Noise & 4.08/28.76 & 35\% &  41\% & 0.7428  \\
& Patch &  3.69/27.57 & 1\% &  100\% & 0.7848 \\
& Watermark &  4.20/28.50 & 5\% & 96\%  & 0.8715  \\
& Logo &  3.41/29.29 & 0 & 100\%  & 0.8234  \\
\bottomrule
\end{tabular}}
\end{table}
